AdaManip: Adaptive Articulated Object Manipulation Environments and Policy Learning

Articulated object manipulation is a critical capability for robots to perform various tasks in real-world scenarios. Composed of multiple parts connected by joints, articulated objects are endowed with diverse functional mechanisms through complex relative motions. For example, a safe consists of a door, a handle, and a lock, where the door can only be opened when the latch is unlocked. The internal structure, such as the state of a lock or joint angle constraints, cannot be directly observed from visual observation. Consequently, successful manipulation of these objects requires adaptive adjustment based on trial and error rather than a one-time visual inference. However, previous datasets and simulation environments for articulated objects have primarily focused on simple manipulation mechanisms where the complete manipulation process can be inferred from the object's appearance. To enhance the diversity and complexity of adaptive manipulation mechanisms, we build a novel articulated object manipulation environment and equip it with 9 categories of objects. Based on the environment and objects, we further propose an adaptive demonstration collection and 3D visual diffusion-based imitation learning pipeline that learns the adaptive manipulation policy. The effectiveness of our designs and proposed method is validated through both simulation and real-world experiments. Our project page is available at: https://adamanip.github.io

==> fig/fig2.tex <==
\begin{figure}
% \centering
\includegraphics[width=1.0\textwidth]{fig/Figure2.pdf}
\caption{
Adaptive manipulation dataset and environments. Bottle and Pressure Cooker feature the \textbf{Rotate \& Slide} mechanism, requiring continued rotation after a failed lift. The window includes the \textbf{Lock} and \textbf{Random Rotation Direction} mechanisms, necessitating exploration of the correct rotation direction to unlock the latch. Microwave incorporates the \textbf{Lock} and \textbf{Switch Contact} mechanisms, where the robot must first pull the handle to check the lock state and press the button if locked.
}
\vspace{-0.5cm}
\label{fig:fig2}
\end{figure}


==> fig/micro_wave_real.tex <==
\begin{figure}
  \vspace{-2mm}
  \centering
  \includegraphics[width=0.85\textwidth]{fig/microwave_real.pdf}
  \caption{Visualization of Open Microwave Experiment in the real world. The red trajectory represents the executed trajectory. In subfigure 2, the blue trajectory indicates the action under the condition that the microwave is unlocked, prompting the robot to continue opening the door.
  }
  \label{fig:fig1}
\vspace{-2mm}
\end{figure}


==> fig/other_cate_real.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[width=0.8\textwidth]{fig/other_catego_real.pdf}
  \caption{Visualization of Open Safe/Bottle/Pressure Cooker Experiment in the real world. The red trajectory represents the executed trajectory. The blue trajectory indicates the actions under the other object state.
  }
  \label{fig:fig1}
\vspace{-4mm}
\end{figure}

==> fig/sim_result.tex <==
\begin{figure}
  % \centering
  % \includegraphics{fig/trails.png}
  \includegraphics[width=1.0\textwidth]{fig/result.pdf}
  \caption{\textbf{Manipulation Trajectories Proposed by Our Method and Others.} Our method can sequentially propose stable and accurate adaptive actions, while others have their respective drawbacks.}
  \label{fig:sim_result}
\end{figure}


==> fig/trails.tex <==
\begin{figure}
  % \centering
  % \includegraphics{fig/trails.png}
  \includegraphics[width=0.9\textwidth]{fig/trails.png}
  \caption{Sample figure caption.}
  \label{fig:trails}
\end{figure}

